Show Me Why It's Correct: Saving 1/3 of Debugging Time in Program Repair with Interactive Runtime Comparison

Automated Program Repair (APR) holds the promise of alleviating the burden of debugging and fixing software bugs. Despite this, developers still need to manually inspect each patch to confirm its correctness, which is tedious and time-consuming. This challenge is exacerbated in the presence of plausible patches, which accidentally pass test cases but may not correctly fix the bug. To address this challenge, we propose an interactive approach called iFix to facilitate patch understanding and comparison based on their runtime difference. iFix performs static analysis to identify runtime variables related to the buggy statement and captures their runtime values during execution for each patch. These values are then aligned across different patch candidates, allowing users to compare and contrast their runtime behavior. To evaluate iFix, we conducted a within-subjects user study with 28 participants. Compared with manual inspection and a state-of-the-art interactive patch filtering technique, iFix reduced participants' task completion time by 36% and 33% while also improving their confidence by 50% and 20%, respectively. Besides, quantitative experiments demonstrate that iFix improves the ranking of correct patches by at least 39% compared with other patch ranking methods and is generalizable to different APR tools.

==> 4-Evaluation.tex <==
To evaluate the overall usefulness and usability of \iFix, we conducted a within-subjects user study with \NumUserStudyParticipants participants that consisted of both college students and professional developers. This study has been approved by the IRB office at the local university. Additionally, to find out to what extent \iFix can help reduce the number of candidate patches to inspect, we conducted quantitative experiments to measure the performance of our {\em patch clustering and sampling} method. We investigate the following research questions:

\begin{itemize}[leftmargin=10mm]
    \setlength\itemsep{0.5mm}
    \item[\textbf{RQ1}] How effectively can \iFix help improve developers' performance in selecting the correct patch from many plausible patches generated by APR techniques? 
    \item[\textbf{RQ2}] To what extent does \iFix improve developers' confidence on automatically generated patches? 
    \item[\textbf{RQ3}] How effective is the {patch clustering and sampling} algorithm in terms of the final rank of the correct patch? 
    % \item[\textbf{RQ4}] How generalizable is the {patch clustering and sampling} algorithm when applied to patches generated by different APR techniques? 
\end{itemize}
